Evolution of the Outflows in NGC 3516

We analyze the 2011 HST/COS spectrum of the Seyfert 1 galaxy NGC 3516, which demonstrates clear changes in one of the intrinsic absorption troughs (component 5), slight evidence of change in a second trough (component 6), and the appearance of a new absorption trough (component 9). We interpret both the changes and the appearance of the new trough as bulk motion across the line of sight. The implied lower limit on the transverse velocity of component 5 is 360 km/s, compared to the earlier 2001 HST/STIS spectrum, while the lower limits for components 6 and 9 are 920 km/s, based on 2009 FUSE data. Component 5 also exhibits a shift in velocity centroid. This is only the second known case of this behavior in a Seyfert galaxy. Due to the high quality of the HST/COS spectrum, we identify a previously undetected trough due to an excited state of Si II for component 1. In combination with the resonance trough of Si II and photoionization modeling, we directly determine the distance of the component 1 outflow to be 67.2 pc.

==> table2b.tex <==
\newpage
\begin{deluxetable}{lcc}
\tablecolumns{3}
\tablewidth{0.6\textwidth}
\tablecaption{Flux Values at 1160 \AA}
\tablehead{
\colhead{Observation Date} &
\colhead{Instrument} & 
\colhead{Flux} \\
\colhead{} &
\colhead{} &
\colhead{(10$^{-15}$ ergs s$^{-1}$ cm$^{-2}$ \AA$^{-1}$)} \\
}

\startdata
2011-01-22 & COS  & 9.74 $\pm$ 1.84 \\
2007-01-23 & FUSE & 24.91 $\pm$ 7.83\\
2006-02-09 & FUSE & 8.18 $\pm$ 1.80 \\
2003-03-29 & FUSE & 3.76 $\pm$ 6.13 \\
2003-01-28 & FUSE & 3.76 $\pm$ 4.97 \\
2002-02-14 & FUSE & 6.08 $\pm$ 3.66 \\
2000-04-17 & FUSE & 5.65 $\pm$ 3.49 \\
\enddata
\normalsize

\end{deluxetable}

